Beyond Gloss: A Hand-Centric Framework for Gloss-Free Sign Language Translation

Sign Language Translation (SLT) is a challenging task that requires bridging the modality gap between visual and linguistic information while capturing subtle variations in hand shapes and movements. To address these challenges, we introduce \textbf{BeyondGloss}, a novel gloss-free SLT framework that leverages the spatio-temporal reasoning capabilities of Video Large Language Models (VideoLLMs). Since existing VideoLLMs struggle to model long videos in detail, we propose a novel approach to generate fine-grained, temporally-aware textual descriptions of hand motion. A contrastive alignment module aligns these descriptions with video features during pre-training, encouraging the model to focus on hand-centric temporal dynamics and distinguish signs more effectively. To further enrich hand-specific representations, we distill fine-grained features from HaMeR. Additionally, we apply a contrastive loss between sign video representations and target language embeddings to reduce the modality gap in pre-training. \textbf{BeyondGloss} achieves state-of-the-art performance on the Phoenix14T and CSL-Daily benchmarks, demonstrating the effectiveness of the proposed framework. We will release the code upon acceptance of the paper.

==> important.tex <==
\subsection{Comparison with State-of-the-Art}
\begin{table*}[!ht]
\tiny
\caption{\small Experimental results on PHOENIX14T dataset. The best results for gloss-free models are highlighted in bold, while the secondbest results are underlined.}
    \centering
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{ lccccc }
    
        % \hline   
        %  \textbf{Method} & \textbf{BLEU1}& \textbf{BLEU2} & \textbf{BLEU3}& \textbf{BLEU4}  & \textbf{ROUGE} \\ \hline
        \hline
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{Test Set}}  \\ \cline{2-6} &\rule{0pt}{1em} \textbf{BLEU-1} & \textbf{BLEU-2} & \textbf{BLEU-3} & \textbf{BLEU-4} & \textbf{ROUGE} \\ \hline

        \rowcolor[HTML]{D2D2D2}
        \multicolumn{6}{c}{\textbf{Gloss-based}} \\ \hline
        MMTLB\cite{mmtlb} &  53.97 & 41.75 & 33.84 & 28.39 & 52.65 \\
        TS-SLT\cite{ts-slt} &  54.90 & 42.43 & 34.46 & 28.95 & 53.48 \\ 
        SLTUNET\cite{sltunet}  & 52.92 & 41.76 & 33.99 & 28.47 & 52.11 \\ 
        \hline
        \rowcolor[HTML]{D2D2D2}
        \multicolumn{6}{c}{\textbf{Gloss-free}} \\ \hline
        NSLT\cite{nslt} &27.10 &15.61 &10.82 &8.35 &29.70\\
        NSLT+Luong\cite{luong} & 29.86 & 17.52 & 11.96 & 9.00 & 30.70 \\
        CSGCR\cite{csgcr} & 36.71 & 25.40 & 18.86 & 15.18 & 38.85 \\
        GFSLT-VLP\cite{gfslt-vlp} & 43.71 & 33.18 & 26.11 & 21.44 & 42.49 \\
        Sign2GPT(w/PGP)\cite{sign2gpt} & \underline{49.54} & \underline{35.96} & \underline{28.83} & 22.52 & \underline{48.90} \\
        FLa-LLM\cite{fla-llm} & 46.29 & 35.33 & 28.03 & \underline{23.09} & 45.27 \\
        LLaVA-SLT\cite{liang2024llavasltvisuallanguagetuning} & 51.20 & 37.51 & 29.39 & 23.43 & 50.44 \\
        
        \cdashline{1-6}
        \textbf{Ours} &\rule{0pt}{1em}\textbf{52.38} & \textbf{38.57} & \textbf{30.74} & \textbf{25.49} & \textbf{51.89} \\
        \hline
    \end{tabular}}
    \label{tab:phinix}
\end{table*}



% \begin{table*}[!t]
% \tiny
% \caption{\small Ablation study on visual encoder on PHOENIX14T.}
% \centering
% \resizebox{0.7\linewidth}{!}{
% \begin{tabular}{cc|cc}
% \hline
% \textbf{Visual Encoder} & \textbf{Trainable} & \textbf{B-4} & \textbf{R} \\ \hline
% ResNet-18& \checkmark  & 18.97 & 40.17   \\
% Dino V2& $\times$ & 20.43 & 42.75   \\
% Dino V2& 3 last layers fine-tuned by LoRA & \textbf{25.49} & \textbf{51.89}\\
% \hline
% \end{tabular}}
% \label{tab:visual}
% \end{table*}



\begin{table*}[!t]
\tiny
\caption{\small Experimental results on Phoenix14T and CSL-Daily datasets. The best results for gloss-free models are highlighted in bold, while the second-best results are underlined.}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccccc|ccccc}
\hline
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{5}{c|}{\textbf{PHOENIX14T}} &
\multicolumn{5}{c}{\textbf{CSL-Daily}} \\
\cline{2-11}
& \textbf{B-1} & \textbf{B-2} & \textbf{B-3} & \textbf{B-4} & \textbf{R}
& \textbf{B-1} & \textbf{B-2} & \textbf{B-3} & \textbf{B-4} & \textbf{R} \\
\hline
\rowcolor[HTML]{D2D2D2}
\multicolumn{11}{c}{\textbf{Gloss-based}} \\ \hline
MMTLB\cite{mmtlb} & 53.97 & 41.75 & 33.84 & 28.39 & 52.65 & 53.31 & 40.41 & 30.87 & 23.92 & 53.25 \\
SLTUNET\cite{sltunet} & 52.92 & 41.76 & 33.99 & 28.47 & 52.11 & 54.98 & 41.44 & 31.84 & 25.01 & 54.08 \\ 
TS-SLT\cite{ts-slt} & 54.90 & 42.43 & 34.46 & 28.95 & 53.48 & 55.44 & 42.59 & 32.87 & 25.79 & 55.72  \\\hline
\rowcolor[HTML]{D2D2D2}
\multicolumn{11}{c}{\textbf{Gloss-free}} \\ \hline
NSLT+Luong\cite{luong} & 29.86 & 17.52 & 11.96 & 9.00 & 30.70 & 34.16 & 19.57 & 11.84 & 7.56 & 34.54 \\
CSGCR\cite{csgcr} & 36.71 & 25.40 & 18.86 & 15.18 & 38.85 & -- & -- & -- & -- & -- \\
GFSLT-VLP\cite{gfslt-vlp} & 43.71 & 33.18 & 26.11 & 21.44 & 42.49 & 39.37 & 24.93 & 16.26 & 11.00 & 36.44 \\
Sign2GPT\cite{sign2gpt} & 49.54 & 35.96 & 28.83 & 22.52 & 48.90 & 41.75 & 28.73 & 20.60 & 15.40 & 42.36 \\
SignCL\cite{signcl} & 49.76 & 36.85 & 29.97 & 22.74 & 49.07 & 47.47 & 32.53 & 22.62 & 16.16 & 48.92 \\
FLa-LLM\cite{fla-llm} & 46.29 & 35.33 & 28.03 & 23.09 & 45.27 & 37.13 & 25.12 & 18.38 & 14.20 & 37.25 \\
SignLLM\cite{signllms} & 45.21  & 34.78 & 28.05 & 23.40 & 44.49 & 39.55 & 28.13 & 20.07 & 15.75 & 39.91 \\
LLaVA-SLT\cite{liang2024llavasltvisuallanguagetuning} & 51.20 & 37.51 & 29.39 & 23.43 & 50.44 & 52.15 & 36.24 & 26.47 & 20.42 & 51.26 \\
\cdashline{1-11}
\textbf{Hand2Sign} & \textbf{52.38} & \textbf{38.57} & \textbf{30.74} & \textbf{25.49} & \textbf{52.89} & \textbf{53.12} & \textbf{38.63} & \textbf{27.82} & \textbf{21.53} & \textbf{53.46} \\
\hline
\end{tabular}}
\label{tab:results}
\end{table*}



\begin{table*}[t]
\tiny
\caption{\small Qualitative results of Phoenix14T. We highlight the difference between sentences.}
\centering
\begin{tabular}{l p{0.6\linewidth}}
\hline
\textbf{Reference:} & am tag wechseln sonne und wolken einander ab teilweise ist es auch langere zeit sonnig. \\
& (During the day sun and clouds alternate partly it is sunny for a long time) \\[1ex]
\textbf{GFSLT-VLP:} & \colorbox{green!30}{am tag wechseln sonne und wolken einander ab} es bilden sich \colorbox{green!30}{langere zeit} viel sonnenschein. \\ & ( During the day, sun and clouds alternate There is a lot of sunshine for a long time )  \\[1ex]
\textbf{Ours:} & \colorbox{green!30}{am tag wechseln sonne und wolken einander ab} zeigt sich die \colorbox{green!30}{auch langere zeit sonnig.} \\ & (During the day, sun and clouds alternate, and the weather remains sunny for longer periods.) \\ \hline
\textbf{Reference:} & am tag nur hier und da einige sonnige momente vor allem an den alpen. \\ & (During the day only here and there some sunny moments, especially in the Alps)\\[1ex]
\textbf{GFSLT-VLP:} & morgen zeigt sich mal die sonne wenn dann \colorbox{green!30}{vor allem an den alpen.} \\ & (Tomorrow the sun will show up , especially in the Alps) \\[1ex]
\textbf{Ours:} & und morgen scheint \colorbox{green!30}{und da einige} die sonnige \colorbox{green!30}{vor allem an den alpen.} \\ & (Tomorrow will shine and there will be some sunny weather, especially in the Alps.) \\ \hline
\textbf{Reference:} & am freitag scheint abseits der nebelgebiete haufig die sonne \\ & (On Friday the sun often shines outside of the foggy areas)\\[1ex]
\textbf{GFSLT-VLP:} & \colorbox{green!30}{am freitag} sobald der nebel weg ist sonnenschein. \\ & (On Friday as soon as the fog is gone there will be sunshine)  \\[1ex]
\textbf{Ours:} & \colorbox{green!30}{am freitag scheint abseits der nebelgebiete haufig die sonne.} \\ & (On Friday the sun often shines outside of the foggy areas) \\ \hline
\end{tabular}
\label{tab:quality}
\end{table*}



% \begin{itemize}
%     \item \textbf{State-of-the-art results:} Our proposed framework, \textbf{Hand2Sign}, achieves state-of-the-art results in gloss-free sign language translation on two widely used benchmark datasets. It surpasses all existing methods in BLEU-4 and ROUGE scores, with particularly notable improvements attributed to emphasizing hands as the primary component of sign language communication.
%     \item \textbf{Hand-focused video descriptions using VLLMs:} We introduce the first method for generating hand-centric textual descriptions of sign language videos using Video Large Language Models (VLLMs), offering a new form of semantic supervision aligned with visual content. 
%     \item \textbf{Leveraging HaMeR feature for SLT:} We are the first to leverage HaMeR’s transformer-based hand representations in the SLT task. Through feature distillation, we guide the visual encoder to focus on hand pose and orientation, demonstrating the positive impact of this strategy on translation quality.  
% \end{itemize}



% \begin{figure}
% \begin{tabular}{ccc}
% \bmvaHangBox{\fbox{\parbox{2.7cm}{~\\[2.8mm]
% \rule{0pt}{1ex}\hspace{2.24mm}\includegraphics[width=2.33cm]{images/eg1_largeprint.png}\\[-0.1pt]}}}&
% \bmvaHangBox{\fbox{\includegraphics[width=2.8cm]{images/eg1_largeprint.png}}}&
% \bmvaHangBox{\fbox{\includegraphics[width=5.6cm]{images/eg1_2up.png}}}\\
% (a)&(b)&(c)
% \end{tabular}
% \caption{. }
% \label{fig:teaser}
% \end{figure}

% Such pre-training strategies can take two forms: pseudo-gloss pretraining and contrastive visual-language pretraining. Pseudo-gloss pretraining generates intermediate text-like representations from sign videos to help the LLMs process them more effectively. Contrastive visual-language pretraining, on the other hand, aligns visual and textual representations by learning a shared feature space, often using contrastive learning techniques to improve modality bridging.
